UnDiFi-2D: an Unstructured Discontinuity Fitting code for 2D grids

UnDiFi-2D, an open source (free software) Unstructured-grid, Discontinuity Fitting code, is presented. The aim of UnDiFi-2D is to model gas-dynamic discontinuities in two-dimensional (2D) flows as if they were true discontinuities of null thickness that bound regions of the flow-field where a smooth solution to the governing PDEs exists. UnDiFi-2D therefore needs to be coupled with an unstructured CFD solver that is used to discretize the governing PDEs within the smooth regions of the flow-field. Two different, in-house developed, CFD solvers are also included in the current distribution. The main features of the UnDiFi-2D software can be summarized as follows: Programming Language: UnDiFi-2D is written in standard Fortran 77/95; its design is highly modular in order to enhance simplicity of use, maintenance and allow coupling with virtually any existing CFD solver; Usability, Maintenance and Enhancement: In order to improve the usability, maintenance and enhancement of the code also the documentation has been carefully taken into account. The git distributed versioning system has been adopted to facilitate collaborative maintenance and code development; Copyrights: UnDiFi-2D is a free software that anyone can use, copy, distribute, change and improve under the GNU Public License version 3. The present paper is a manifesto of the first public release of the UnDiFi-2D code. It describes the currently implemented features, which are the result of more than a decade of still ongoing CFD developments. This work is focused on the computational techniques adopted and a detailed description of the main characteristics is reported. UnDiFi-2D capabilities are demonstrated by means of examples test cases. The design of the code allows to easily include existing CFD codes and is aimed at ease code reuse and readability.

==> SE.tex <==
\subsection{Unsteady test-case: Shock-expansion interaction\label{subsec:SE}}
This test case deals with an expansion fan interacting with a moving shock. The present calculations have been performed using the \texttt{NEO} code both in shock-capturing and shock-fitting mode. The problem involves a rectangular cavity initially filled with an inviscid perfect gas at rest, as shown in the sketch of Fig.~\ref{fig:P1P2}a. The left end of the domain acts as a piston which is impulsively set into motion, generating a planar shock wave moving towards the closed (right) end of the domain. Given the density ratio across the shock wave, all other kinematic and thermodynamic quantities follow from the Rankine--Hugoniot (R-H) jump relations and are summarized in Table~\ref{tab:IC}. The upstream and downstream dimensionless quantities have been labelled with the subscripts 1 and 2 in Table~\ref{tab:SE}. The Mach number in a reference frame attached to the shock is denoted by $M_r$, and its upstream value coincides with that of the dimensionless shock speed $W_s$, since $a_1$ has been chosen as the reference velocity. After the impulsive startup, the piston starts slowing down at $t=t_0+t_s$; its velocity and position are prescribed analytically by:

\begin{equation}
u_{p}\left(t\right)=\begin{cases}
u_{2}^{*}          & t_0<t<0 \\
u_{2}\exp^{-t} & t\ge 0
\end{cases},
\qquad x_{p}
\left(t\right)=\begin{cases}
u_{2}t & t_0<t<0\\
u_{2}t\left(1-\exp^{-t}\right) & t\ge 0
\end{cases}\label{piston_velocity}
\end{equation}
where $t_0=-t_s$ and:
\begin{equation}
t_{s}=\frac{x_{sh}^{0}}{W_{s}-u_{2}}\simeq0.3755
\label{eq:tshock}
\end{equation}

The flow evolution is sketched in the $x - t$ plane of Fig.~\ref{fig:P3}. We start the simulations at $t=0$ with the shock located $x_{sh}^{0}=0.3$ unit lengths ahead of the piston and we initialize the solution using the initial conditions listed in Table~\ref{tab:SE}. The tail of the expansion wave (marked by arrows in Fig.~\ref{fig:P3} is the straight, characteristic line of slope $u_2+a_2$ that is shed from the origin of the space-time plane and divides the expansion wave from the uniform, shock-downstream region, labelled 2 in Fig.~\ref{fig:P1P2}. Up to time:

\begin{equation}
\hat{t}=\frac{x_{sh}^{0}}{(u_{2}+a_{2})-W}=\frac{x_{sh}^{0}}{(1-M_{r,2})a_2}\simeq0.8339
\label{eq:tfinal}
\end{equation}
when the tail of the expansion wave meets the shock trajectory, the expansion region is a simple wave, so that an analytical solution can be computed as described, for instance, in~\cite{salas20091st}. At later times, the expansion wave is reflected off the moving shock as an expansion wave of the opposite family, the shock starts reducing its speed and the region of the $x-t$ plane that is between the moving piston and the moving shock ceases to be a simple wave.
%\begin{figure}[H]
%\centering
%\includegraphics[scale=0.75]{figs/SE_1.png}
%\caption{Shock-expansion interaction. (a) Computational set-up at $t=0$. (b) Nested meshes and shock position at $t=2.8$. (c) Pressure iso-contours in the space-time plane.}
%\label{fig:SE1} 
%\end{figure}
\begin{figure}[H]
\centering
\includegraphics[scale=0.3]{figs/piston1.png}
\includegraphics[scale=0.3]{figs/piston2.png}
\caption{Shock-expansion interaction. (a) Computational set-up at $t=0$. (b) Nested meshes and shock position at $t=2.8$. %(c) Pressure iso-contours in the space-time plane.
}
\label{fig:P1P2} 
\end{figure}
\begin{figure}[H]
\centering
\includegraphics[scale=0.3]{figs/piston3.png}
\caption{Shock-expansion interaction: %(a) Computational set-up at $t=0$. (b) Nested meshes and shock position at $t=2.8$. 
pressure iso-contours in the space-time plane.}
\label{fig:P3} 
\end{figure}

\begin{center}
\begin{table}[H]
\caption{Shock-expansion interaction: initial conditions.}
\label{tab:SE}
\begin{centering}
\begin{tabular}{ccccccc}
\hline 
 & $\rho$ & $u$ & $v$ & $p$ & $M_r$ & $a$\tabularnewline
\hline 
\hline 
Upstream (1) & 1.4 & 0.0 & 0.0 & 1.0 & 1.5336 & 1\tabularnewline
\hline 
Downstream (2) & 2.6872 & 0.7346 & 0.0 & 2.5772 & 0.6895 & 1.1588\tabularnewline
\hline 
\end{tabular}
\par\end{centering}
\end{table}
\par\end{center}
Simulations have been advanced until the final time $t=2.8$ when the shock is located at $x_{sh}^{t_2} = 4.43$ and has almost reached the closed (right) end of the cylinder. We present results obtained on a background grid of 639 nodes, 12448 triangles, with a shock front discretized by 41 points (cfr. right picture of Fig.~\ref{fig:P1P2}a). During the time evolution, the streamwise size of the computational domain is reduced because of the piston's motion. All nodes of the background mesh move as the time elapses, but the topology of the mesh does not change. At any time instant, the location of the nodes of the background mesh is prescribed using the following equation:
\begin{equation}
x_{i}\left(t\right)=x_{i}\left(0\right) + x_{p}\left(t\right)\left(1-\frac{x_{i}\left(0\right)}{L}\right)
\label{eq:pistonlaw}
\end{equation}
where $L=5$ is the streamwise length of the computational domain at $t=0$.

Figure~\ref{fig:pcontour} provides the pressure field at three subsequent time instants for all the five different spatial discretization schemes selected in \texttt{NEO} and the two shock-modelling schemes. Apart from the excessive shock-thickness of the shock-capturing solutions, it is clear that shock-fitting provides a much cleaner representation of the shock-downstream region. Observe, in particular, that the cross-flow non-uniformities are considerably less pronounced in the shock-fitting calculations. 

Figure~\ref{fig:pline} shows the streamwise pressure profiles at two subsequent time instants for all the five spatial discretization schemes. Note that the figures report all the data points in the mesh. The superiority of the shock-fitting calculations is evident, particularly in the reduction of cross-shock spurious variations, despite the fact that both the fitted and captured solutions are represented on unstructured triangulations with almost identical topologies. We do observe an impact of the numerical discretization chosen. The upwind or centred nature of the method does not seem to affect the results as much as the resolution of the scheme. The N scheme clearly provides the "wrong boundary conditions" for the shock, which seems slightly misplaced w.r.t. the analytical solution, as one can see in the right frame of Fig.~\ref{fig:pline}a. Shock amplitude and position are instead perfectly matched by the high order schemes, with perhaps a barely visible off-set present only in the LDAN result, shown in Fig.~\ref{fig:pline}c. These differences are clearly much more important in the captured solutions: the linear, first-order-accurate N scheme smears the shock-profile over a considerable streamwise extent; as expected, the linear, second-order-accurate, but non-monotone LDA and SU schemes give rise to overshoots around the discontinuity; the non-linear, second-order-accurate LDAN scheme is monotonicity preserving, but the otherwise similar Bc scheme also overshoots the shock profile.
\begin{figure}[H]
\centering
\includegraphics[scale=0.75]{figs/SE_2.png}
\caption{Shock-expansion interaction: pressure contours at times $t=0.4$ (left), $t=1.2$ (centre) and $t=2.0$ (right): 20 equally spaced contour levels between 0.5 and 2.6, fitted solutions on top and captured solutions on the bottom of each frame. (a) $t=0.4$ N scheme. (b) $t=1.2$ N scheme. (c) $t=2.0$ N scheme. (d) $t=0.4$ LDA scheme. (e) $t=1.2$ LDA scheme. (f) $t=2.0$ LDA scheme. (g) $t=0.4$ LDAN scheme. (h) $t=1.2$ LDAN scheme. (i) $t=2.0$ LDAN scheme. (j) $t=0.4$ SU scheme. (k) $t=1.2$ SU scheme. (l) $t=2.0$ SU scheme. (m) $t=0.4$ Bc scheme. (n) $t=1.2$ Bc scheme. (o) $t=2.0$ Bc scheme.}
\label{fig:pcontour} 
\end{figure}

\begin{figure}[H]
\centering
\includegraphics[scale=1.1]{figs/SE_3.png}
\caption{Shock-expansion interaction: streamwise pressure profiles at two time instants for all the five spatial discretization schemes. Right column: zoom of the $t=2.8$ peak. (a) N scheme. (b) LDA scheme. (c) LDAN scheme. (d) SU scheme. (e) Bc scheme.}
\label{fig:pline} 
\end{figure}
